Part2Object: Hierarchical Unsupervised 3D Instance Segmentation

Unsupervised 3D instance segmentation aims to segment objects from a 3D point cloud without any annotations. Existing methods face the challenge of either too loose or too tight clustering, leading to under-segmentation or over-segmentation. To address this issue, we propose Part2Object, hierarchical clustering with object guidance. Part2Object employs multi-layer clustering from points to object parts and objects, allowing objects to manifest at any layer. Additionally, it extracts and utilizes 3D objectness priors from temporally consecutive 2D RGB frames to guide the clustering process. Moreover, we propose Hi-Mask3D to support hierarchical 3D object part and instance segmentation. By training Hi-Mask3D on the objects and object parts extracted from Part2Object, we achieve consistent and superior performance compared to state-of-the-art models in various settings, including unsupervised instance segmentation, data-efficient fine-tuning, and cross-dataset generalization. Code is release at https://github.com/ChengShiest/Part2Object

==> tables/sc_new_table.tex <==

\newcommand{\fig}[2][1]{\includegraphics[width=#1\linewidth]{#2}}
\newcommand{\figh}[2][1]{\includegraphics[height=#1\linewidth]{fig/#2}}
\newcommand{\figa}[2][1]{\includegraphics[width=#1]{fig/#2}}
\newcommand{\figah}[2][1]{\includegraphics[height=#1]{fig/#2}}

\begin{tabular}{ccccc}
\multicolumn{5}{c}{\fig[.99]{figs/vis/s1.png}} \\
\multicolumn{5}{c}{\fig[.99]{figs/vis/s2.png}} \\
\multicolumn{5}{c}{\fig[.99]{figs/vis/s3.png}} \\
\phantom{1500} Input  &\phantom{37000} Felzenswalb~\cite{felzenszwalb2004efficient}  &\phantom{600} CutLER~\cite{wang2023cut} & \phantom{10000}Ours  &\phantom{700} GT\\

% \fig[.20]{figs/vis/l1.png} &
% \fig[.20]{figs/vis/l2.png}  &
% \fig[.20]{figs/vis/l3.png}  &
% \fig[.20]{figs/vis/l4.png}  &
% \fig[.20]{figs/vis/l5.png}  \\


% \rotatebox{90}{\phantom{600} Input} & \fig[.99]{figs/vis/s1.png} \\
% \rotatebox{90}{ Felzenswalb~\cite{felzenszwalb2004efficient}} &\fig[.99]{figs/vis/s2.png} \\
% \rotatebox{90}{ CutLER~\cite{wang2023cut}} &\fig[.99]{figs/vis/s3.png} \\


% \fig[.24]{figs/vis/0081_01/scene0081_01_vh_clean_2.png} &
% \fig[.24]{figs/vis/0355_00/scene0355_00_vh_clean_2.png}  &
% \fig[.24]{figs/vis/0427_00/scene0427_00_vh_clean_2.png}  &
% \fig[.24]{figs/vis/0609_00/scene0609_00_vh_clean_2.png}  \\

% \fig[.24]{figs/vis/0081_01/0081_01_f.png} &
% \fig[.24]{figs/vis/0355_00/0355_00_f.png}  &
% \fig[.24]{figs/vis/0427_00/0427_00_f.png}  &
% \fig[.24]{figs/vis/0609_00/0609_00_f.png}  \\

% \fig[.24]{figs/vis/0081_01/scene0081_01_merge_ncut.png} &
% \fig[.24]{figs/vis/0355_00/scene0355_00_merge_ncut.png}  &
% \fig[.24]{figs/vis/0427_00/scene0427_00_merge_ncut.png}  &
% \fig[.24]{figs/vis/0609_00/scene0609_00_merge_ncut.png}  \\

% \fig[.24]{figs/vis/0081_01/scene0081_01_plabel.png} &
% \fig[.24]{figs/vis/0355_00/scene0355_00_plabel.png}  &
% \fig[.24]{figs/vis/0427_00/scene0427_00_plabel.png}  &
% \fig[.24]{figs/vis/0609_00/scene0609_00_plabel.png}  \\

% \fig[.24]{figs/vis/0081_01/scene0081_01.png} &
% \fig[.24]{figs/vis/0355_00/scene0355_00.png}  &
% \fig[.24]{figs/vis/0427_00/scene0427_00.png}  &
% \fig[.24]{figs/vis/0609_00/scene0609_00.png}  \\





\end{tabular}

==> tables/tab2_p2_s3dis.tex <==
\begin{tabular}{lrrrrrr}\toprule
\multicolumn{1}{c}{} &\multicolumn{6}{c}{mAP@50 S3DIS ~\cite{s3dis}}  \\\cmidrule(lr){2-7} 
Methods &Area 1 &Area 2 &Area 3 &Area 4 &Area 5  &Area 6\\\midrule
Mask3D~\cite{Schult23mask3d}  & 12.4 & 10.6 &13.1 &10.9&11.5 & 11.6 \\
\rowcolor{gray} Ours & 17.1 & 16.4 & 16.6  & 17.0& 14.1 & 17.6 \\
\bottomrule
\end{tabular}

==> tables/tab2_p2_scannet200.tex <==
\begin{tabular}{lcccccc}\toprule
\multicolumn{1}{c}{} &\multicolumn{3}{c}{mAP@50 ScanNet200 Val~\cite{dai2017scannet}} &\multicolumn{3}{c}{mAP@25} \\\cmidrule(lr){2-7} 
Methods &Head &Common &Tail&Head &Common &Tail\ \ \  \\\midrule
Mask3D~\cite{Schult23mask3d}   & 20.3 &19.5 & 18.7& 26.7 &26.0 & 23.6\\

\rowcolor{gray} Ours  & 32.2 & 30.5 & 24.5& 60.8 &53.8 & 45.2\\
\bottomrule
\end{tabular}

==> tables/table1.tex <==
\begin{table}[t]
    % \small
    \centering
    \label{tbl:table1}
    \caption{Ablation study on the clustering algorithm, with the top sub-table focused on pseudo-label generation strategies and the bottom on the Hi-Mask3D network architecture.}
    \begin{tabular}{lccc}
        \toprule
         & AP & AP@25 & AP@50  \\
        \midrule
        Direct Clustering & 6.1  & 37.8 & 13.8 \\
         w/o Object Guidance & 10.4 & 43.2 & 20.7 \\
         w/o Feature Update & 10.6 & 44.2 & 21.5  \\
        Ours Pseudo labels  & \textbf{12.6}& \textbf{55.1} & \textbf{26.8} \\
        \midrule
        Train with Mask3D & 14.2 & 59.0 & 31.0  \\
        Train with Hi-Mask3D  & \textbf{16.9} & \textbf{64.9} & \textbf{36.0} \\
        \bottomrule
    \end{tabular} 
    \label{tab3}
\end{table}

==> tables/table2.tex <==

% \begin{table*}[htbp]
%     \centering
%     % \tiny
%     \caption{table 2}
    
%     \renewcommand\arraystretch{1.25}
%     % \tabcolsep=0.5cm
%     \label{tbl:table2}
%     % \setlength{\tabcolsep}{3mm}{
%     % \resizebox{\textwidth}{20mm}{
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{c|ccc|c|c|c|c}
%         \hline 
%         \multirow[b]{2}{*}{ Model } & \multicolumn{3}{c}{ Unsupervised } & \multicolumn{1}{c}{ 1\% } & \multicolumn{1}{c}{ 5\% } & \multicolumn{1}{c}{ 10\% } & \multicolumn{1}{c}{ 20\% } \\
%         % \cmidrule(lr){3-5}\cmidrule(lr){6}\cmidrule(lr){7}\cmidrule(lr){8}\cmidrule(lr){9}\cmidrule(lr){10}
%          & AP@25 & AP@50 &  AP  & AP@50 & AP@50 &  AP@50  & AP@50 \\
%         \hline 
%         HDBSCAN & 32.1 & 5.5 & 1.6 & - & - & - & - \\
%         Nunes et al. & 30.5 & 7.3 & 2.3 & - & - & - & - \\
%         Felzenswalb & 38.9 & 12.7 & 5.0 & - & - & - & - \\
%         CutLER Projection  & 7.0 & 0.2 & 0.3 & - & - & - & -\\
%         Scratch & - & - & - & 14.1 & 33.3 & 39.2 & 43.4 \\
%         CSC  & - & - & - & 22.1 & 39.9 & 43.8 & 48.9 \\
%         Unscene3D & 58.5 & 32.2 & 15.9 & 28.4 & 46.8 & 55.7 & 60.7\\
%         \textbf{Ours} & \textbf{69.0} & \textbf{37.3} & \textbf{17.4} & \textbf{44.1} & \textbf{64.2} & \textbf{68.0} & \textbf{72.1} \\
%         \hline
%         \end{tabular}
%     }
%     % }
%     % }
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{main table}
% \label{tab:nuscenes_semkitti}
% \scalebox{1.0}{
% \begin{tabular}{r|p{1.06cm}<{\centering}p{1.06cm}<{\centering}p{1.06cm}<{\centering}|p{1.14cm}<{\centering}|p{1.14cm}<{\centering}|p{1.14cm}<{\centering}|p{1.14cm}<{\centering}}
% \toprule
% \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Unsupervised}} \vline & \textbf{1\%} & \textbf{5\%} & \textbf{10\%} & \textbf{20\%}
% \\
% & \textcolor{gray}{\textbf{AP@25}} & \textcolor{gray}{\textbf{AP@50}} & \textcolor{gray}{\textbf{AP}} & \textcolor{gray}{\textbf{AP@50}} & \textcolor{gray}{\textbf{AP@50}} & \textcolor{gray}{\textbf{AP@50}} & \textcolor{gray}{\textbf{AP@50}}
% \\\midrule
% % \cellcolor{yellow!8}Random & \cellcolor{yellow!8}$56.15$ & \cellcolor{yellow!8}$65.48$ & \cellcolor{yellow!8}$74.66$ & \cellcolor{yellow!8}$39.50$ & \cellcolor{yellow!8}$39.41$ & \cellcolor{yellow!8}$20.22$
% % \\
% % PointContrast~{\small\textcolor{gray}{[ECCV'20]}}  & - & - & - & $41.10$ & - & -
% % \\
% % DepthContrast~{\small\textcolor{gray}{[ICCV'21]}}  & - & - & - & $41.50$ & - & -
% % \\
% % PPKT~{\small\textcolor{gray}{[arXiv'21]}}  & $60.25$ & $67.14$ & $74.52$ & $44.00$ & $47.60$ & $61.10$
% % \\
% % SLidR~{\small\textcolor{gray}{[CVPR'22]}}  & $59.84$ & $66.91$ & $74.79$ & $44.60$ & $47.12$ & $63.10$
% % \\
% % ST-SLidR~{\small\textcolor{gray}{[CVPR'23]}}  & $60.75$ & $67.70$ & $75.14$ & $44.72$ & $44.93$ & -
% % \\

%         HDBSCAN & $32.1$ & $5.5$ & $1.6$ & - & - & - & - \\
%         Nunes et al. & $30.5$ & $7.3$ & $2.3$ & - & - & - & - \\
%         Felzenswalb & $38.9$ & $12.7$ & $5.0$ & - & - & - & - \\
%         CutLER Projection  & $7.0$ & $0.2$ & $0.3$ & - & - & - & -\\
%         Scratch & - & - & - & $14.1$ & $33.3$ & $39.2$ & $43.4$ \\
%         CSC  & - & - & - & $22.1$ & $39.9$ & $43.8$ & $48.9$ \\
%         Unscene3D & $58.5$ & $32.2$ & $15.9$ & $28.4$ & $46.8$ & $55.7$ & $60.7$\\
% \cellcolor{violet!7}Ours & \cellcolor{violet!7}$\mathbf{69.0}$ & \cellcolor{violet!7}$\mathbf{37.3}$ & \cellcolor{violet!7}$\mathbf{17.4}$ & \cellcolor{violet!7} $\mathbf{44.1}$& \cellcolor{violet!7}$\mathbf{64.2}$ & \cellcolor{violet!7}$\mathbf{68.0}$ & \cellcolor{violet!7}$\mathbf{72.1}$ \\
% % \\\midrule
% % \textbf{Seal~$^\dagger$ {\small(Ours)}} & $65.52$ & $70.80$ & $77.13$ & -& - & -
% % \\
% % \textbf{Seal~$^\ddagger$ {\small(Ours)}} & $66.78$ & $72.31$ & $78.28$ & - & - & -
% % \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

% \begin{table}[htbp]
%     \centering
%     % \tiny
%     % \renewcommand\arraystretch{1.25}
%     % \tabcolsep=0.5cm
%     \label{tbl:table1}
%     \setlength{\tabcolsep}{2mm}{
%     % \resizebox{\textwidth}{20mm}{
%     \begin{tabular}{llccc}
%         \Xhline{1pt}
        
%         &Method & AP@ & AP@25 & AP@50 \\
        
%         \Xhline{1pt}
%         \multirow{6}{*}{w/o training}
%         &HDBSCAN & $1.6$  & $32.1$ & $5.5$ \\
%         &Nunes et al. & $2.3$  & $30.5$ & $7.3$ \\
%         &Felzenswalb & $5.0$  & $38.9$ & $12.7$\\
%         &CutLER  & $0.3$  & $7.0$& $0.2$\\
%         &Unscene3D & $5.9$  & $19.9$& $10.0$\\
%         &\cellcolor{violet!7}\textbf{Ours} & \cellcolor{violet!7}$\mathbf{12.6}$  & \cellcolor{violet!7}$\mathbf{55.1}$  & \cellcolor{violet!7}$\mathbf{26.8}$\\
%         \Xhline{1pt}
%         \multirow{3}{*}{self-training}
%         &FreePoint & $10.7$  & $37.8$ & $21.4$\\
%         &Unscene3D & $15.9$ & $58.5$ & $32.2$\\
% &\cellcolor{violet!7}\textbf{Ours} & \cellcolor{violet!7}$\mathbf{16.9}$  & \cellcolor{violet!7}$\mathbf{64.9}$& \cellcolor{violet!7}$\mathbf{36.0}$ \\

 
%         \Xhline{1pt}
%     \end{tabular} 
%     \caption{Results of Unsupervised Setting}
%     \label{tab1}
%     }
%     % }
% \end{table}


% \begin{table}[htbp]
%     \centering
%     % \small
%     % \renewcommand\arraystretch{1.25}
%     % \tabcolsep=0.5cm
%     \label{tbl:table1}
%     \setlength{\tabcolsep}{2.5mm}{
%     % \resizebox{\textwidth}{20mm}{
%     \begin{tabular}{lccc}
%         \toprule
%         Method & AP & AP@25 & AP@50 \\
%         \midrule
%         HDBSCAN~\cite{mcinnes2017accelerated_hdbscan} & $1.6$  & $32.1$ & $5.5$ \\
%         Nunes et al.~\cite{nunes2022unsupervised} & $2.3$  & $30.5$ & $7.3$ \\
%         Felzenswalb~\cite{felzenszwalb2004efficient} & $5.0$  & $38.9$ & $12.7$\\
%         CutLER~\cite{wang2023cut}  & $0.3$  & $7.0$& $0.2$\\
%         Unscene3D~\cite{rozenberszki2023unscene3d} & $5.9$  & $19.9$& $10.0$\\
%         \cellcolor{violet!7}\textbf{Ours} & \cellcolor{violet!7}$\mathbf{12.6}$  & \cellcolor{violet!7}$\mathbf{55.1}$  & \cellcolor{violet!7}$\mathbf{26.8}$\\
%         \bottomrule
%     \end{tabular} 
%     \caption{Model performance under unsupervised setting. }
%     \label{tab1}
%     }
%     \vspace{-3mm}
%     % }
% \end{table}


==> tables/table3.tex <==
\begin{table}[htbp]
    \centering
    % \tin
    \renewcommand\arraystretch{1.25}
    % \tabcolsep=0.5cm
    % \setlength{\tabcolsep}{3mm}{
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{l|ccc}
        \Xhline{2pt}
        \multirow{2}{*}{ScanNet~\cite{dai2017scannet} $\rightarrow$ ScanNet200~\cite{rozenberszki2022language}} & Head & Common & Tail \\
&  \textcolor{gray}{\textbf{AP@50}} & \textcolor{gray}{\textbf{AP@50}} & \textcolor{gray}{\textbf{AP@50}} \\
        
        % Scannet200 & AP & AP@50 & AP@25 \\ 
        \hline
        
        Mask3D~\cite{Schult23mask3d} (fully supervised) & 29.4 & 26.3 & \textbf{25.6} \\
        \textbf{Ours} (unsupervised) & \textbf{31.0} & \textbf{29.2} & 23.1 \\
        \Xhline{1.5pt}
        ScanNet~\cite{dai2017scannet} $\rightarrow$ S3DIS~\cite{armeni2017joint}  & AP & AP@50 & AP@25 \\ 
        \hline
        Mask3D~\cite{Schult23mask3d} (fully supervised) &\textbf{13.1} & 19.2 &  26.0 \\
        \textbf{Ours}(unsupervised) & 11.5 & \textbf{23.9} & \textbf{39.2} \\
        % \Xhline{1.5pt}
        % dataset & AP & AP@50 & AP@25 \\ 
        % \hline
        % supervised model 1& 30 & 30 & 30 \\ 
        % supervised model 2& 30 & 30 & 30 \\
        % supervised model 3& 30 & 30 & 30 \\
        % \textbf{Ours} & \textbf{20} & \textbf{20} & \textbf{20} \\
        \Xhline{2pt}
    \end{tabular} 
    }
    \caption{Cross-dataset Generalization Results on S3DIS~\cite{armeni2017joint} and ScanNet200~\cite{rozenberszki2022language}.}
    \label{supp}
    % }
    % }
\end{table}



==> tables/table_ab_part.tex <==
\begin{table}[htbp]
    \centering
    % \tiny
    % \renewcommand\arraystretch{1.25}
    % \tabcolsep=0.5cm
    \label{tbl:table1}
    % \setlength{\tabcolsep}{3mm}{
    % \resizebox{\textwidth}{20mm}{
    \begin{tabular}{lccc}
        \Xhline{1pt}
        
         & AP@25 & AP@50 & AP \\
        
        \Xhline{1pt}
        Mask3D~\cite{Schult23mask3d} & 32.1 & 5.5 & 1.6 \\
        Hi-Mask3D w/o $\mathcal{L}_{c}$ & 30.5 & 7.3 & 2.3 \\
        Ours & \textbf{58.5} & \textbf{32.2} & \textbf{15.8} \\

 
        \Xhline{1pt}
    \end{tabular} 
    \caption{Ablation Study on part2Obj}
    % }
    % }
\end{table}

==> tables/table_ab_self.tex <==
\begin{table}[htbp]
    % \small
    \centering

    \setlength{\tabcolsep}{2mm}{
    % \resizebox{\textwidth}{20mm}{
    \begin{tabular}{lccc}
        \toprule
         & AP@25 & AP@50 & AP \\
        \midrule
        Pseudo labels  & 55.1 & 26.8 & 12.6 \\
        $1^{st}$ Self-Training  & 60.7 & 32.6 & 15.3 \\
        $2^{nd}$ Self-Training & 64.3 & 35.2 & 16.5 \\
        $3^{rd}$ Self-Training & \textbf{64.9} & \textbf{36.0} & \textbf{16.9} \\
        \bottomrule
    \end{tabular} 
    \caption{Ablation study on self-training.}
    \label{tab4}
    }
    % }
    \vspace{-4mm}
\end{table}

==> tables/table_on_data_efficient_.tex <==
\begin{table}[t]
% \small
\centering
\setlength{\tabcolsep}{1.5mm}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Method}} & \textbf{0\%}  & \textbf{1\%} & \textbf{5\%} & \textbf{10\%} & \textbf{20\%}
\\ 

\cmidrule{2-6} 
&  \multicolumn{5}{c}{\textcolor{gray}{AP@50}} \\
\midrule
        Scratch & - & $14.1$ & $33.3$ & $39.2$ & $43.4$ \\
        CSC~\cite{hou2021exploring} & - & $22.1$ & $39.9$ & $43.8$ & $48.9$ \\
        Unscene3D~\cite{rozenberszki2023unscene3d} & 23.2 & $28.4$ & $46.8$ & $55.7$ & $60.7$\\
\cellcolor{violet!7}\textbf{Ours} & \cellcolor{violet!7}$\mathbf{32.6}$ & \cellcolor{violet!7} $\mathbf{44.1}$& \cellcolor{violet!7}$\mathbf{64.2}$ & \cellcolor{violet!7}$\mathbf{68.0}$ & \cellcolor{violet!7}$\mathbf{72.1}$ \\

\bottomrule
\end{tabular}
}
\caption{Model performance under data-efficient setting.}
\label{tab2}
\vspace{-5mm}
\end{table}

==> tables/temp.tex <==
\begin{tabular}{lccc}\toprule
\multicolumn{1}{c}{w/o training} &\multicolumn{3}{c}{ScanNet Val~\cite{dai2017scannet}}  \\\cmidrule(lr){2-4} 
Methods &mAP@25 &mAP@50 &mAP\ \ \  \\\midrule
HDBSCAN~\cite{mcinnes2017accelerated_hdbscan}  & 1.6 & 32.1 &5.5 \\
Nunes~\cite{nunes2022unsupervised} & 2.3 & 30.5 & 7.3\\
Felzenswalb~\cite{felzenszwalb2004efficient} & 5.0 & 38.9 & 12.7 \\
CutLER~\cite{wang2023cut} & 0.3 & 7.0 & 0.2 \\
Unscene3D~\cite{rozenberszki2023unscene3d} & 5.9 & 19.9 & 10.0 \\
Ours & 2.6 & 55.1 & 26.8 \\
\bottomrule
\end{tabular}
